Nanoscale Three-Dimensional Imaging of Integrated Circuits using a Scanning Electron Microscope and Transition-Edge Sensor Spectrometer

X-ray nanotomography is a powerful tool for the characterization of nanoscale materials and structures, but is difficult to implement due to competing requirements on X-ray flux and spot size. Due to this constraint, state-of-the-art nanotomography is predominantly performed at large synchrotron facilities. We present a laboratory-scale nanotomography instrument that achieves nanoscale spatial resolution while changing the limitations of conventional tomography tools. The instrument combines the electron beam of a scanning electron microscope (SEM) with the precise, broadband X-ray detection of a superconducting transition-edge sensor (TES) microcalorimeter. The electron beam generates a highly focused X-ray spot in a metal target held micrometers away from the sample of interest, while the TES spectrometer isolates target photons with high signal-to-noise. This combination of a focused X-ray spot, energy-resolved X-ray detection, and unique system geometry enable nanoscale, element-specific X-ray imaging in a compact footprint. The proof-of-concept for this approach to X-ray nanotomography is demonstrated by imaging 160 nm features in three dimensions in 6 layers of a Cu-SiO2 integrated circuit, and a path towards finer resolution and enhanced imaging capabilities is discussed.

==> instructions.tex <==
\section*{Instructions for Editing (omit for preprint)}
Authors:  please copy the two ``new commands'' above with your initials.  Pick a color.  Please use your initial in capitals to suggest a text insertion.  Please use your text in lower case to comment on the text in italics.

Please use $\backslash$\textrm{todonotes[inline]$\{\dots\}$.  If you don't say ``inline'', the comment goes on the right and the text gets small.}

$\backslash$\textrm{sout \sout{is also available}}.

\NJN{Sample suggested text.}
\njn{Sample comment on text}

